Comparison of PBO solvers in a dependency solving domain

Linux package managers have to deal with dependencies and conflicts of packages required to be installed by the user. As an NP-complete problem, this is a hard task to solve. In this context, several approaches have been pursued. Apt-pbo is a package manager based on the apt project that encodes the dependency solving problem as a pseudo-Boolean optimization (PBO) problem. This paper compares different PBO solvers and their effectiveness on solving the dependency solving problem.

==> eptcsdata.tex <==
\providecommand{\event}{I. Lynce and R. Treinen (eds.): Workshop on\\
Logics for Component Configuration (LoCoCo 2010)}
\providecommand{\volume}{29}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{23}
\providecommand{\eid}{3}
\providecommand{\publicationstatus}{I. Lynce and R. Treinen (eds.): Workshop on\\
Logics for Component Configuration (LoCoCo 2010)\\
EPTCS 29, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.29.3}{10.4204/EPTCS.29.3}}
\pdfoutput=1

